Easily parallelizable and distributable class of algorithms for structured sparsity, with optimal acceleration

Many statistical learning problems can be posed as minimization of a sum of two convex functions, one typically a composition of non-smooth and linear functions. Examples include regression under structured sparsity assumptions. Popular algorithms for solving such problems, e.g., ADMM, often involve non-trivial optimization subproblems or smoothing approximation. We consider two classes of primal-dual algorithms that do not incur these difficulties, and unify them from a perspective of monotone operator theory. From this unification we propose a continuum of preconditioned forward-backward operator splitting algorithms amenable to parallel and distributed computing. For the entire region of convergence of the whole continuum of algorithms, we establish its rates of convergence. For some known instances of this continuum, our analysis closes the gap in theory. We further exploit the unification to propose a continuum of accelerated algorithms. We show that the whole continuum attains the theoretically optimal rate of convergence. The scalability of the proposed algorithms, as well as their convergence behavior, is demonstrated up to 1.2 million variables with a distributed implementation.

==> sections/algorithms.tex <==
\section{Two primal-dual algorithm classes}\label{sec:main}
We introduce the two classes of algorithms to study. Note the first-order optimality condition for \eqref{eqn:primal} is given by
\begin{subequations}\label{eqn:optimality}
\begin{align}
	0 &= \nabla f(x^{\star}) + K^T y^{\star}, \label{eqn:optimality1}\noeqref{eqn:optimality1} \\
	y^{\star} &\in \partial h(Kx^{\star}). \label{eqn:optimality2}
\end{align}
\end{subequations}
%where $\partial h(u)$ is the subdifferential of the convex function $h(\cdot)$ at $u \in \mathbb{R}^l$.
The inclusion condition \eqref{eqn:optimality2} is equivalent to
	$Kx^{\star} \in (\partial h)^{-1}(y^{\star}) = \partial h^{*}(y^{\star})$,
which is the optimality condition for the following optimization problem
\[
	\text{minimize}\quad h^{*}(v) + (2\sigma)^{-1}\| v - y^{\star} - \sigma K x \|_2^2,
\]
for any $\sigma >0$. That is,
%\[
	$y^{\star} = \prox_{\sigma h^{*}} ( y^{\star} + \sigma Kx^{\star})$.
%\]
Thus we obtain an alternative formulation of the optimality condition in the form of a fixed-point equation:
\begin{align}
\begin{split}\label{eqn:fixedpoint}
	x^{\star} &= x^{\star} - \tau(\nabla f(x^{\star}) + K^T y^{\star}),  \\
	y^{\star} &= \prox_{\sigma h^{*}} ( y^{\star} + \sigma Kx^{\star}), 
\end{split}
\end{align}
for $\tau, \sigma >0$.
Throughout, we assume a solution $(x^\star, y^\star)$ to \eqref{eqn:optimality} and \eqref{eqn:fixedpoint} exists. 
%
Under a suitable assumption made precise in Section \ref{sec:main}, the minimization problem \eqref{eqn:primal} can be equivalently written as the following saddle-point problem 
\begin{align}\label{eqn:saddlepoint}
		\min_{x\in\mathbb{R}^p} \max_{y\in\mathbb{R}^l} f(x) + \langle Kx, y \rangle - h^{*}(y),
\end{align}
where
$h^{*}(v) = \sup_{u \in \mathbb{R}^l} \langle u, v \rangle - h(u)$
is the convex conjugate of $h$;
$\langle u,v \rangle$ denotes the standard inner product $u^Tv$.
%
Then, \eqref{eqn:primal} is equivalent to \eqref{eqn:saddlepoint}, $(x^\star, y^\star)$ satisfies the saddle-point condition for \eqref{eqn:saddlepoint}:
\[
	\mathcal{L}(x^{\star},y) \le\mathcal{L}(x^{\star},y^{\star}) \le\mathcal{L}(x,y^{\star}), \quad \forall x \in \mathbb{R}^n,~ \forall y \in \mathbb{R}^l,
\]
where the saddle function
$\mathcal{L}(x,y) = f(x) + \langle Kx, y \rangle - h^{*}(y)$
is convex in $x$ and concave in $y$, and $y^\star$ is a solution to the dual problem of \eqref{eqn:primal}.
Thus %both Algorithms LV and CO are primal-dual algorithms, in which $x$ is the primal and
$y$ can be interpreted as the dual variable.

The two classes of algorithms that we study solve the saddle-point problem \eqref{eqn:saddlepoint} iteratively. 
%The algorithms of our study solve \eqref{eqn:fixedpoint} iteratively. 
The first class is due to  \citet{loris2011generalization}, \citet{Chen:InverseProblems:2013}, and \citet{drori2015simple}:
\begin{align*}\tag{Algorithm LV}
\begin{split}\label{eqn:LV}\noeqref{eqn:LV}
    \tilde{x}^{k+1} &= x^k - \tau \left(\nabla f(x^k) + K^T y^k\right) \\
    %y^{k+1} &= \prox_{\sigma h^{*}} \left( y^k + \sigma K \tilde{x}^{k+1}\right)
	%\tag{Algorithm LV}
	%\\
    %x^{k+1} &= \tilde{x}^{k+1} - \tau K^T(y^{k+1}-y^{k}),
	y^{k+1} &= (1-\rho_k) y^k + \rho_k \prox_{\sigma h^{*}}(y^k + \sigma K \tilde{x}^{k+1}) \\
	x^{k+1} &= (1-\rho_k) x^k + \rho_k (\tilde{x}^{k+1} - \tau K^T(y^{k+1}-y^{k})),
\end{split}
\end{align*}
%and its relaxed variant
%\begin{align*}
%y^{k+1} &= (1-\rho_k) y^k + \rho_k \prox_{\sigma h^{*}}(y^k + \sigma K \tilde{x}^{k+1}) \\
%x^{k+1} &= (1-\rho_k) x^k + \rho_k (\tilde{x}^{k+1} - \tau K^T(y^{k+1}-y^{k})),
%\end{align*}
where 
the sequence $\{\rho_k\} \subset [0,\delta]$ satisfies $\sum_{k=0}^{\infty}\rho_k(\delta-\rho_k)=\infty$ with $\delta \allowbreak = \allowbreak 2-(\tau L_f)/(2-2\sigma\tau\|K\|_2^2)$; 
$\prox_{\phi}(z) \allowbreak := \allowbreak \argmin_{z' \in \mathbb{R}^n} \phi(z') + \frac{1}{2}\| z' - z \|_2^2$ is the proximity operator for a convex function $\phi$.
The sequence $\{(x^k,y^k)\}$ generated by this iteration converges to a solution $(x^{\star},y^{\star})$ to \eqref{eqn:saddlepoint}, if exists, for $(\sigma,\tau)$ with %such that
\begin{align}\label{eqn:LVparamrange}
	%\frac{1}{\tau} > \frac{L_f}{2} \quad \text{and} \quad \frac{1}{\tau\sigma} > \|K\|_2^2.
	1/\tau > L_f/2 \quad \text{and} \quad 1/(\tau\sigma) > \|K\|_2^2.
\end{align}
Algorithm LV is similar to the Combettes-Pesquet method \eqref{eqn:CP} of Section \ref{sec:related}, but requires one \replaced{fewer}{less} step per iteration with an additional step size parameter $\sigma$. 
%Its inertial variant is considered in Section \ref{sec:rates}.
The second class is due to \citet{Condat:JournalOfOptimizationTheoryAndApplications:2012} and \citet{Vu2013}:%, which originally considers a three-function extension of \eqref{eqn:primal} that minimizes $f(x) + g(x) + h(Kx)$ with $g$ closed, proper, and convex:
\begin{align*}\tag{Algorithm CV}
\begin{split}\label{eqn:CV}\noeqref{eqn:CV}
    %x^{k+1}         &= \prox_{\tau g} \left( x^k - \tau \left(\nabla f(x^k) + K^T y^k\right) \right) \;\; & \\
    \bar{x}^{k+1} &= x^k - \tau(\nabla f (x^k) + K^T y^k)\\
    \tilde{x}^{k+1} &= 2x^{k+1} - \bar{x}^{k+1} \\
    x^{k+1} &= (1-\rho_k) x^k + \rho_k \bar{x}^{k+1} \\
    %y^{k+1}         &= \prox_{\sigma h^{*}} (y^k + \sigma K \tilde{x}^{k+1}),&
    y^{k+1} &= (1-\rho_k) y^k + \rho_k \prox_{\sigma h^{*}} (y^k + \sigma K \tilde{x}^{k+1}),
\end{split}
\end{align*}
%and its relaxed version as that for Algorithm LV,
% \begin{align*}
%     \overline{x}^{k+1}         &= x^k - \tau \left(\nabla f(x^k) + K^T y^k\right) \;\; & \\
%     \tilde{x}^{k+1} &= 2 \overline{x}^{k+1} - x^k \\
%     y^{k+1} &= (1-\rho_k) y^k + \rho_k \prox_{\sigma h^{*}} (y^k + \sigma K \tilde{x}^{k+1}) \\
%     x^{k+1} &= (1-\rho_k) x^k + \rho_k \overline{x}^{k+1},
% \end{align*}
which converges for $(\sigma,\tau)$ such that
\begin{align}\label{eqn:CPparamrange2}
	%\frac{1}{\tau} > \frac{L_f}{2} \quad \text{and} \quad \left(\frac{1}{\tau}-\frac{L_f}{2}\right)\frac{1}{\sigma} > \|K\|_2^2.
	1/\tau > L_f/2 \quad \text{and} \quad \left(1/\tau-L_f/2\right)/\sigma > \|K\|_2^2.
\end{align}
This condition is slightly more restrictive than \eqref{eqn:LVparamrange}. %In problem \eqref{eqn:primal}, $g \equiv 0$, and the $\prox_{\tau g}$ in the first line disappears. %; an inertial variant is also considered in Section \ref{sec:rates}. 
%Algorithm CV is related to another three-function-sum minimization method by \citet{Combettes2012}. 
%In the two-function case, 
Algorithm CV can be considered as a variant of the PDHG \eqref{eqn:pdhg} where the evaluation of $\prox_{\tau f}$, which can be costly, is replaced by that of $I - \tau \nabla f$.%; see Appendix \ref{sec:related} for details.



==> sections/derivation.tex <==

\section{Derivation of preconditioned forward-backward splitting algorithms}\label{sec:derivation}
\subsubsection*{Algorithm LV}
Write Algorithm LV as
\begin{align}
    x^{k+1} &= x^k - \tau \left(\nabla f(x^k) + K^T y^{k+1}\right) \label{eqn:LV1} \\
    (I+\sigma\partial h^{*})(y^{k+1}) &\ni y^k + \sigma K \tilde{x}^{k+1} \nonumber \\
									&= y^k + \sigma K(I-\tau\nabla f)(x^k) - \sigma\tau KK^Ty^k \nonumber \\
									&= \sigma K (I-\tau\nabla f)(x^k) + (I-\sigma\tau KK^T)y^k \label{eqn:LV2}
\end{align}
Left-multiply $\sigma K$ to both sides of \eqref{eqn:LV1} and subtract from \eqref{eqn:LV2} to obtain
\begin{align}\label{eqn:LV2-2}
	-\sigma K x^{k+1} + (I-\sigma\tau KK^T + \sigma\partial h^{*})(y^{k+1}) \ni (I-\sigma\tau KK^T)y^k
\end{align}
Combine \eqref{eqn:LV1} and \eqref{eqn:LV2-2} to write
\begin{align}\label{eqn:LVsplit}
	\begin{bmatrix} \frac{1}{\tau}I & K^T \\ -K & \frac{1}{\sigma}I-\tau KK^T + \partial h^{*} \end{bmatrix}
	\begin{bmatrix} x^{k+1} \\ y^{k+1} \end{bmatrix}
	\ni
	\begin{bmatrix} \frac{1}{\tau}I-\nabla f &   \\    & \frac{1}{\sigma}I-\tau KK^T \end{bmatrix}
	\begin{bmatrix} x^{k} \\ y^{k} \end{bmatrix}
\end{align}
Let
\begin{align*}%\label{eqn:LVoperators}
	M_{\mathsf{LV}} = \begin{bmatrix} \frac{1}{\tau}I &  \\  & \frac{1}{\sigma}I-\tau KK^T \end{bmatrix},
	\quad
	F = \begin{bmatrix} 0 & K^T \\ -K & \partial h^{*} \end{bmatrix},
	\quad
	G = \begin{bmatrix} \nabla f & 0 \\ 0 & 0 \end{bmatrix}.
\end{align*}
Then we see that \eqref{eqn:LVsplit} is
\begin{align*}
	(M_{\mathsf{LV}}+F)(z^{k+1}) \ni (M_{\mathsf{LV}}-G)(z^k),
\end{align*}
where $z^k=(x^k,y^k)$, which in turn is equivalent to
\begin{align}\label{eqn:LVfb}
	z^{k+1} = (I+M_{\mathsf{LV}}^{-1}F)^{-1}(I-M_{\mathsf{LV}}^{-1}G)(z^k).
\end{align}
Note that $F+G=T$, where $T$ is given in \eqref{eqn:inclusion}, the optimality condition for \eqref{eqn:objective}.

\subsubsection*{Algorithm CV}
Write Algorithm CV as
\begin{align}
    x^{k+1} &= x^k - \tau \left(\nabla f(x^k) + K^T y^{k}\right) \label{eqn:CP1} \\
    (I+\sigma\partial h^{*})(y^{k+1}) &\ni y^k + \sigma K \tilde{x}^{k+1} \nonumber \\
									&= y^k + \sigma K(2x^{k+1}-x^k) \nonumber \\
									&= y^k - \sigma K x^k + 2\sigma K x^{k+1} \label{eqn:CP2},
\end{align}
Inclusion \eqref{eqn:CP2} is equivalent to
\begin{align}\label{eqn:CP2-2}
	-2\sigma K x^{k+1} + (I + \sigma \partial h^{*})(y^{k+1}) \ni -\sigma K x^k + y^k
\end{align}
Combine \eqref{eqn:CP1} and \eqref{eqn:CP2-2} to write
\begin{align}\label{eqn:CPsplit}
	\begin{bmatrix} \frac{1}{\tau}I & 0 \\ -2K & \frac{1}{\sigma}I + \partial h^{*} \end{bmatrix}
	\begin{bmatrix} x^{k+1} \\ y^{k+1} \end{bmatrix}
	\ni
	\begin{bmatrix} \frac{1}{\tau}I-\nabla f & -K^T   \\ -K  & \frac{1}{\sigma}I \end{bmatrix}
	\begin{bmatrix} x^{k} \\ y^{k} \end{bmatrix}
\end{align}
Let
\begin{align}\label{eqn:CPoperators}
	M_{\mathsf{CV}} = \begin{bmatrix} \frac{1}{\tau}I & -K^T \\ -K  & \frac{1}{\sigma}I \end{bmatrix},
	\quad
	F = \begin{bmatrix} 0 & K^T \\ -K & \partial h^{*} \end{bmatrix},
	\quad
	G = \begin{bmatrix} \nabla f & 0 \\ 0 & 0 \end{bmatrix}.
\end{align}
Then we see that \eqref{eqn:CPsplit} is
\begin{align*}
	(M_{\mathsf{CV}}+F)(z^{k+1}) \ni (M_{\mathsf{CV}}-G)(z^k),
\end{align*}
where $z^k=(x^k,y^k)$, which in turn is equivalent to
\begin{align*}%\label{eqn:CPfb}
	z^{k+1} = (I+M_{\mathsf{CV}}^{-1}F)^{-1}(I-M_{\mathsf{CV}}^{-1}G)(z^k).
\end{align*}
Note that the operators $F$ and $G$ are the same as Algorithm LV.
%Thus $F+G=T$, where $T$ is given in \eqref{eqn:inclusion}, the optimality condition for \eqref{eqn:objective}.
%Thus Algorithm CV is a preconditioned forward-backward splitting algorithm with preconditioner $M_{\mathsf{CV}}$ and splitting given in \eqref{eqn:CPoperators}.





% \section{Visualization of region of convergence for $C = \kappa K$} \label{sec:vis}
% Figure \ref{fig:paramrange} visualizes the region of convergence given by \eqref{eqn:generalparamrange} for $C = \kappa K$, for various values of $\kappa$. We can see that the smaller $|\kappa|$ is, the wider the corresponding region of convergence is.
% \begin{figure}[H]
% \vskip 0.2in
% \begin{center}
% \centerline{
% \def\svgwidth{0.7\columnwidth}
% \input{paramrange.pdf_tex}
% }
% \caption{Range of convergence for $1/\sigma$ and $1/\tau$. Boundaries correspond to $|\kappa|$ = 0, 0.25, 0.5, 0.75, 1.}
% \label{fig:paramrange}
% \end{center}
% \vskip -0.2in
% \end{figure}


==> sections/distributed.tex <==
\section{Feature-splitting distributed computation}\label{sec:dist}


Algorithms LV, CV, and \eqref{eqn:accgen} preferably with sparse $K$, only consist of elementwise operations, matrix-vector multiplications and proximity operators, and they do not require quadratic minimization. Hence they are suitable for distributed processing, provided that $\prox_{\sigma h^{*}}(\cdot)$ is separable in the partitions. As illustrated in Table \ref{tab:examples}, this is indeed the case for many statistical learning problems.

We consider the case that the number of features $p$ is so large that, for each sample, the features do not fit into the memory. In other words, the data matrix
$A = [A^{[1]}, \dotsc, A^{[M]} ]$, where $A^{[i]} \in \mathbb{R}^{n \times p_i}$, $\quad \sum_{i=1}^m p_i = p$,
is stored distributedly in $M$ machines. In this case, it is desirable  to also split the vectors $x \in \mathbb{R}^p$ conformally and store distributedly, i.e., $x = [x_{[1]}^T, \dotsc, x_{[M]}^T]^T$, $x_{[i]} \in \mathbb{R}^{p_i}$. For many instances of \eqref{eqn:primal} including the generalized lasso and group lasso, $l \gtrsim p$, so it is desirable to partition and store the dual variable $y \in \mathbb{R}^l$ likewise. i.e., $y = [y_{[1]}^T, \dotsc, y_{[M]}^T]^T$, $y_{[i]} \in \mathbb{R}^{l_i}$, $\sum_{i=1}^m l_i = l$.  To compute $K^T y$ and $Kx$ efficiently, it is desirable to also distribute rows and columns of $K$ across the machines, i.e., $K^T = [K_{[1]}^T, \dotsc, K_{[M]}^T]$ and $K = [K^{[1]}, \dotsc, K^{[M]}]$, where $K_{[i]} \in \mathbb{R}^{l_i \times p}$, and $K^{[i]} \in \mathbb{R}^{l \times p_i}$.  Duplicating $K$ does not incur too much cost, as $K$ is typically sparse. Then, we can carry out computation in a distributed fashion.  e.g., using a scatter-gather model, as long as  machine $i$ has an access to $A_{[i]}$, $K_{[i]}$, and $K^{[i]}$. In such case, communication cost for multiplication with $A$ or $A^T$ is $O(mn)$. When the number of nonzero elements in $K$ is $O(p)$, which is the case for examples in Table \ref{tab:examples}, the communication cost for multiplication with $K$ and $K^T$ is $O(p)$.  
This model is especially suitable for multi-GPU platforms. Many recent GPU programming packages including Theano \cite{theano}, TensorFlow \cite{tensorflow}, and PyTorch \cite{pytorch} deals with inter-GPU communications internally, so that the programmers do not need to implement such communications. %In Appendix \ref{sec:distalgo}, we provide an example for Algorithm LV.
% Deduce the iteration
% \begin{align}\label{eqn:distributedfixedpointiteration}
% 	\bar\beta_j^{(t+1)} &= \beta_j^{(t)} - X_j^Tr^{(t)} - d_j^{(t)}, \quad j=1,\dotsc, N,  \nonumber \\
% 	\bar\gamma_j^{(t+1)} &= \sum_{k=1}^N D_{jk}\bar\beta_k^{(t+1)}, \quad j=1,\dotsc, N, \nonumber \\
% 	\begin{bmatrix} w_1^{(t+1)} \\ \vdots \\ w_N^{(t+1)} \end{bmatrix}
% 	&= \prox_{H^{*}}\left(
% 	\begin{bmatrix} w_1^{(t)} + \bar\gamma_1^{(t+1)} \\ \vdots \\ w_N^{(t)} + \bar\gamma_N^{(t+1)}  \end{bmatrix}
% 	\right), \nonumber \\
% 	d_j^{(t+1)} &= \sum_{k=1}^N D_{kj}^T w_k^{(t+1)}, \quad j=1,\dotsc, N,  \\
% 	\beta_j^{(t+1)} &= \beta_j^{(t)} - X_j^Tr^{(t)} - d_j^{(t+1)}, \quad j=1,\dotsc, N,  \nonumber \\
% 	z_j^{(t+1)} &= X_j \beta_j^{(t+1)}, \quad j=1,\dotsc, N, \nonumber \\
% 	r^{(t+1)} &= l'(\sum_{j=1}^N z_j^{(t+1)}, y). \nonumber
% \end{align}
% where
% $$
% l'(z,y) = \begin{bmatrix} l'_1(z_1,y_1) \\ \vdots \\ l'_n(z_n,y_n) \end{bmatrix}.
% $$



==> sections/inertial.tex <==
\subsection{Inertial variant}\label{sec:inertial}

For the inertial variant \eqref{eqn:inertial}, we present an $O(1/N)$ ergodic rate with minimal assumptions.

\begin{theorem}\label{thm:inertialergodic}
	Let $M$ be the symmetric, positive definite matrix in iteration \eqref{eqn:inertial} and $\mu$ satisfy \eqref{eqn:normupperbound}.
	Write $z^{k}=(x^{k},y^{k})$, $\tilde{z}^{k}=(\tilde{x}^{k},\tilde{y}^{k})$.
	Let $\bar{x}^{N} = (1/N)\sum_{k=1}^N x^{k}$ and $\bar{y}^{N} = (1/N)\sum_{k=1}^N y^{k}$.
	If $\mu > L_f/2$ and
	a nondecreasing sequence $\{\beta_k\} \subset [0,\beta]$, $\bar\beta \le 1/3$, is chosen so that there exists an $\eta > 0$ with
	\begin{align}\label{eqn:inertialcond}
		(1-3\beta_k-\eta) M \succeq \frac{(1-\beta_k)^2}{2}\begin{bmatrix} L_f I &  \\  & 0 \end{bmatrix},
	\end{align}
	for all $k$,
	then for the sequence $\{z^k\}$ generated by \eqref{eqn:inertial} with $z^0 = z^{-1} \in \mathbb{R}^p \times \mathbb{R}^l$,
	the following holds:
	%TODO: alignment
	\begin{align*}
		\MoveEqLeft[2] \mathcal{L}(\bar{x}^N,y) - \mathcal{L}(x,\bar{y}^N) 
		\le \frac{1-\beta_0}{2N}\left( \|z^{0}-z\|_M^2 + \frac{2(1+\bar\beta)^2L_f}{9(1-\bar\beta)\eta\lambda_{\min}(M)}\|z^{0}-z^{\star}\|_M^2\right),
	\end{align*}
	where $z^{\star}$ is a point in $\zer{(F+G)}$.
\end{theorem}


Again by Proposition \ref{prop:Mcondition}, the condition for Theorem \ref{thm:inertialergodic} is equivalent to
	%Condition \eqref{eqn:normupperbound} for $\mu > L_f/2$ implies that
	\eqref{eqn:Mbound} in Theorem \ref{thm:nonergodic}
	for some $\nu > L_f/2$ and $\epsilon > 0$.
	Thus condition \eqref{eqn:inertialcond} is satisfied if
	\[
		(1-3\beta_k-\eta)\begin{bmatrix} \nu I &  \\   & \epsilon I \end{bmatrix}
		\succeq
		\frac{(1-\beta_k)}{2}^2\begin{bmatrix} L_f I &  \\  & 0 \end{bmatrix}.
	\]
	In other words, the inertial version \eqref{eqn:inertial} of \eqref{eqn:preconditionedforwardbackward_} (hence those of Algorithms LV and CV) converges at $O(1/N)$ ergodic rate for any $\eta \in (0,(9-4L_f/\nu)/(L_f/\nu))$,
	if $\{\beta_k\}$ is nondecreasing with $0\le \beta_k \le \bar\beta$ where
	\[
		\bar\beta = \min\left( \frac{1-\eta}{3}, 1 - \frac{3-\sqrt{9-4(L_f/\nu)-2\eta(L_f/\nu)}}{L_f/\nu} \right).
	\]
	This condition is almost identical to that of \citet{Lorenz:JournalOfMathematicalImagingAndVision:2015}, under which \eqref{eqn:inertial} converges but the rate is missing, except for a slight loss of the upper bound from $(1+\eta)/3$ to $(1-\eta)/3$.

 For the inertial variant of Algorithm CV % (and CV+),
 the same $O(1/N)$ ergodic rate is given \cite{Chambolle:MathematicalProgramming:2015}, for a more restrictive range than above (With a strong convexity assumption on $f$ and $h^*$, a linear convergence rate is obtained; see also \citet{Bot2014, Bot2015a}).
The rate of convergence analysis for the inertial variant of Algorithm LV appears to be the first in the literature.%\subsubsection*{Comments}
%\begin{remark}
%When $\beta_k\equiv 0$, i.e., no inertia, condition \eqref{eqn:inertialcond} is equivalent to \eqref{eqn:fullrange}.
%\end{remark}

\begin{remark}
There is a more sophisticated variant of Algorithm CV that achieves the optimal rate \cite{chen2014optimal}.
		Whether the same optimal rate can be attained for a similar variant of Algorithm LV, or more generally, \eqref{eqn:preconditionedforwardbackward_} with the family of preconditioners $M$ given in \eqref{eqn:generalM} would be an interesting outlet for the future research.
\end{remark}



==> sections/related.tex <==
\section{\added[remark={Section Moved}]{Related Methods}}\label{sec:related}
There are various existing methods that can be applied to solving the problem \eqref{eqn:primal}. 
Here, we briefly summarize several most relevant ones.
%\subsubsection*{Proximal gradient method}
\paragraph{Proximal gradient method.}
The proximal gradient method is a forward-backward splitting algorithm applied to the primal \eqref{eqn:primal}.
\deleted{The first-order optimality condition \eqref{eqn:optimality} is given by \eqref{eqn:firstorderopt}.}%for \eqref{eqn:primal} is %without introducing the dual variable $y$ is
Letting $F=K^T\circ\partial h\circ K$ (maximally monotone) and $G=\nabla f$ ($1/L_f$-cocoercive, see Appendix \ref{sec:theory}) and applying forward-backward splitting
%\begin{align}
%z^{k+1} = R_{tF} (I - tG) (z^k)
%\end{align}
, we obtain
	$x^{k+1} = \prox_{th\circ K}(x^{k}-t\nabla f(x^{k})) = \argmin_{x} f(x^{k}) + \langle \nabla f(x^{k}), x-x^{k} \rangle + \frac{1}{2t}\|x-x^{k}\|_2^2 + h(Kx)$
which converges for $0 < t < 2/L_f$.
When $h(\cdot)=\lambda\|\cdot\|_1$ and $K=I$, this is the celebrated iterative shrinkage-thresholding algorithm \citep[ISTA,][]{Beck:SiamJournalOnImagingSciences:2009}.
For this particular $h$ and $K$ being a discrete difference matrix on a graph (fused lasso), evaluating $\prox_{t h\circ K}(v)$ is equivalent to solving the fused lasso signal approximator \citep[FLSA,][]{Friedman:TheAnnalsOfAppliedStatistics:2007} that minimizes
	$\frac{1}{2}\|x-v\|_2^2 + t\lambda \|Kx\|_1$,
for which efficient methods have been proposed \cite{liu2010efficient,xin2014efficient}.

However, for general $K$ and other choices of $h$, e.g., group lasso, evaluation of $\prox_{t h\circ K}$ is not trivial. In this case, approximating $h$ by a smooth function can be considered \cite{Nesterov:MathematicalProgramming:2004}.
\citet{Chen:TheAnnalsOfAppliedStatistics:2012} propose to approximate %$h^{*}(y)$ by $\tilde{h}_{\mu}^{*}(y)=h^{*}(y)+(\mu/2)\|y\|_2^2$. This is equivalent to approximate
$h(x)$ by its Moreau-Yosida smoothing $\tilde{h}_{\mu}(x) = \inf_{u+v=x} h(u) + \frac{1}{2\mu}\|v\|_2^2$.
In particular, when $h(x)=\lambda\|x\|_1$, $\tilde{h}_{\mu}(x)$ is the Huber function \cite{Huber:RobustStatistics:1981}.
Because $\tilde{h}_{\mu}$ is differentiable and $\nabla\tilde{h}_{\mu}$ is Lipschitz continuous (with constant $1/\mu$), the proximal gradient method is applicable. 
\citet{yu2015high} propose to approximate $h(Kx)$ by a quadratic majorizing function locally and iteratively minimize the sum of the majorizing function and $f(x)$. Although this approach is not precisely a proximal gradient method, it falls into the category of majorization-minimization (MM) methods \added[remark={AE, Minor comment 2}]{\citep[see e.g.,][]{lange2000optimization}} that include the proximal gradient as a special case.

%\subsubsection*{Alternating directions method of multipliers (ADMM)}
\paragraph{Alternating directions method of multipliers (ADMM).}
ADMM \citep[see, e.g.,][]{Boyd:FoundationsAndTrendsInMachineLearning:2010} solves \eqref{eqn:primal} using the augmented Lagrangian
$\mathcal{L}_t(x,\tilde{x},y) = f(x) + h(\tilde{x}) + \langle y, Kx-\tilde{x} \rangle + (t/2)\|Kx-\tilde{x}\|_2^2$
in a manner similar to the Gauss-Seidel iteration:
\begin{subequations}\label{eqn:ADMM}
\begin{align}
	x^{k+1} &= \argmin_x \mathcal{L}_t(x,\tilde{x}^{k},y^{k})= \argmin_x f(x) + (t/2)\|Kx-\tilde{x}^{k}+(1/t)y^{k}\|_2^2 \label{eqn:ADMM:x} \\
	\tilde{x}^{k+1} &= \argmin_{\tilde{x}} \mathcal{L}_t(x^{k+1},\tilde{x},y^{k}) = \prox_{(1/t)h}(K x^{k+1}+(1/t)y^{k})\label{eqn:ADMM:b} \\
		 	%= \argmin_{\tilde{x}} h(\tilde{x}) + (t/2)\|Kx^{k+1}-\tilde{x}+(1/t)y^{k}\|_2^2 \nonumber\\
	y^{k+1} &= y^{k} + t (Kx^{k+1}-\tilde{x}^{k+1})\label{eqn:ADMM:c}\noeqref{eqn:ADMM:c}
\end{align}
\end{subequations}
The $x$-update \eqref{eqn:ADMM:x} is potentially expensive to compute. For example, if $f(x)=\frac{1}{2}\|\mathsf{A}x-b\|_2^2$, then the corresponding update involves solving a linear equation of the form $(\mathsf{A}^T\mathsf{A} + t K^TK)x=r$.
While $K$ is structured and known \textit{a priori}, $\mathsf{A}$ is data-dependent in regression problems hence the matrix $\mathsf{A}^T\mathsf{A} + tK^TK$ is hardly structured. %This is the key difference from the image processing problems in which $F$ models the pixel degradation process.
\citet{Ye:ComputationalStatisticsDataAnalysis:2011} propose to solve \eqref{eqn:ADMM:x} iteratively using the preconditioned conjugate gradient method.

ADMM \eqref{eqn:ADMM} for \eqref{eqn:primal} is equivalent to the Douglas-Rachford operator splitting method applied to the Fenchel dual \cite{eckstein1992} : %of \eqref{eqn:primal}:
\begin{align}\label{eqn:dual}
	\text{minimize} ~  h^{*}(y) + f^{*}(-Ky).
\end{align}
The Douglas-Rachford splitting utilizes the equivalence of $0 \in \zer{(F+G)}$ to $z=R_{tG}(\tilde{z})$ with $\tilde{z} \in \Fix{(2R_{tF}-I)(2R_{tG}-I)}$.
This relation suggests a KM iteration $\tilde{z}^{k+1}=\frac{1}{2}\tilde{z}^{k} + \frac{1}{2}(2R_F-I)(2R_G-I)\tilde{z}^{k}$, $z^{k+1}=R_G(\tilde{z}^{k+1})$. It can be shown that by applying this iteration to \eqref{eqn:dual} with $F=\partial h^{*}$ and $G=(-K)^T\circ\partial f^{*}\circ(-K)$, \eqref{eqn:ADMM} is obtained. % (XXX cite Boyd ADMM book XXX).
Note that evaluation of $R_{tG}(v)=\prox_{tf^{*}\circ(-K)}(v)$ is not straightforward; this is connected to the difficulty with \eqref{eqn:ADMM:x}.

\paragraph{Linearized ADM (LADM).}
\added[remark={Reviewer 1, Point 2}]{One may further linearize} the quadratic terms in \eqref{eqn:ADMM:x} and \eqref{eqn:ADMM:b}, and add a proximal term to each of them to replace the quadratic term with a proximity operator \citep{lin2011linearized}:
\begin{subequations}\label{eqn:LADMM}
\begin{align}
\begin{split}\label{eqn:LADMM:x}\noeqref{eqn:LADMM:x}
	x^{k+1} &= \argmin_x f(x) + \langle K^T (y^k)+ t K^T (K x^k - \tilde{x}^k), x - x^k \rangle + (t s_A/2)\| x - x^k \|_2^2 \\
	&= \prox_{(1/(t s_A) f} (x^k - \frac{1}{t s_A}K^T (y^k + t (K x^k - y^k)))  
\end{split}\\
	\tilde{x}^{k+1} &= \prox_{1/(t s_B) h} (\tilde{x}^k + \frac{1}{ts_B}(y^k + t (Kx^{k+1} - \tilde{x}^k)) \label{eqn:LADMM:b}\noeqref{eqn:LADMM:b} \\
		 	%= \argmin_{\tilde{x}} h(\tilde{x}) + (t/2)\|Kx^{k+1}-\tilde{x}+(1/t)y^{k}\|_2^2 \nonumber\\
	y^{k+1} &= y^{k} + t (Kx^{k+1}-\tilde{x}^{k+1})\label{eqn:LADMM:c}\noeqref{eqn:LADMM:c}.
\end{align}
\end{subequations}
This algorithm converges if $s_A > \|K\|_2^2$ and $s_B>1$.  

%\subsubsection*{Primal-dual hybrid gradient method (PDHG)}
\paragraph{Primal-dual hybrid gradient method (PDHG).}
\added[remark={Reviewer 2, Minor comment 4}]{PDHG was first introduced by \citet{zhu2008efficient}, but its convergence was not guaranteed. Its modification due to \citet{Esser:SiamJournalOnImagingSciences:2010}, which introduces} \eqref{eqn:pdhg:xtilde}:
\deleted{PDHG \cite{zhu2008efficient,Esser:SiamJournalOnImagingSciences:2010} is the following iteration} %MODIFIEDFROM:\cite{zhu2008efficient,Esser:SiamJournalOnImagingSciences:2010}
\begin{subequations}\label{eqn:pdhg}
\begin{align}
    x^{k+1}         &= \prox_{\tau f}(x^k - \tau K^T y^k ) \label{eqn:pdhg:x} \\
    \tilde{x}^{k+1} &= 2 x^{k+1} - x^k \label{eqn:pdhg:xtilde}\\
    y^{k+1}         &= \prox_{\sigma h^{*}} (y^k + \sigma K \tilde{x}^{k+1})\label{eqn:pdhg:y}\noeqref{eqn:pdhg:y},
\end{align}
\end{subequations}
converges if $\sigma, \tau >0$ and $\sigma\tau\|K\|_2^2 < 1$ \replaced[remark={Reviewer 2, Minor Comment 5}]{\cite{chambolle2011first,He:SiamJournalOnImagingSciences:2012,Chambolle:MathematicalProgramming:2015}}{\cite{chambolle2011first,He:SiamJournalOnImagingSciences:2012}}.
%Note its resemblance with Algorithm CO. This method also has an advantage that $f$ needs not smooth.
Note that evaluation of $\prox_{th\circ K}$ is replaced by $\prox_{\sigma h^{*}}$, which is usually simpler; see Section \ref{sec:main} for examples.
Nevertheless, similar to ADMM, when $f$ is data-dependent, $\prox_{\tau f}(v)$ is difficult to evaluate:
if $f(x)=\frac{1}{2}\|\mathsf{A}x-b\|_2^2$, then \eqref{eqn:pdhg:x} involves solving a linear equation of the form $(tI + \mathsf{A}^T\mathsf{A})x=r$.

PDHG can be motivated from several approaches. In particular, \eqref{eqn:pdhg} can be obtained from ADMM applied to the Fenchel dual \eqref{eqn:dual}:
% (hence the Douglas-Rachford splitting applied to the primal \eqref{eqn:primal})
\begin{align*}
	\tilde{y}^{k+1} &= \prox_{(1/\tau)f^{*}}((1/\tau)x^{k}-K^Ty^{k}) \\
	x^{k+1} &= x^{k} + \tau (K^Ty^{k}+\tilde{y}^{k+1})  \\
	y^{k+1} &= \argmin_{y} h^{*}(y) + (\tau/2)\|K^Ty+z^{k+1}-(1/\tau)x^{k+1}\|_2^2
\end{align*}
by adding an additional regularization term $\frac{1}{2}\|y-y^{k}\|_{(1/\sigma)I-\tau KK^T}^2$ to the minimization problem in the $y$-update \cite{Esser:SiamJournalOnImagingSciences:2010,chambolle2011first,zhu2015augmented}.

\paragraph{Combettes-Pesquet method \citep{Combettes2012}.}
The Combettes-Pesquet method is a forward-backward-forward operator splitting (see \citet{Bauschke:ConvexAnalysisAndMonotoneOperatorTheoryIn:2011}), % applied to the three-function-sum problem as Algorithm CV:
yielding the following iteration:
\begin{align}
\begin{split}\label{eqn:CP}
\tilde{x}^{k+1} &=  x^k - \tau(\nabla f (x^k) + K^T y^k ) \\
\tilde{y}^{k+1} &= \prox_{\tau h^*} (y^k + \tau K x^k) \\
x^{k+1} &= \tilde{x}^{k+1} - \tau K^T (\tilde{y}^{k+1} - y^k) \\
y^{k+1} &= \tilde{y}^{k+1} + \tau K (\tilde{x}^{k+1}-x^k).
\end{split}
\end{align}
The algorithm converges for $\tau \in [\epsilon, (1-\epsilon)/\beta]$, where $\beta = L_f + \|K\|_2$ and  $\epsilon \in (0, 1/(\beta+1))$.


==> sections/stoc.tex <==
\section{Stochastic Algorithm}
\subsection{Algorithm}
In this subsection, we present an algorithm to solve Problem \eqref{eqn:saddle} by a class of iterative algorithms similar to \eqref{eqn:accgen} which acquire the approximate solutions via a subsequent calls to a stochastic oracle($\mathcal{SO}$). On the $t$-th call, the oracle returns the stochastic gradient $(\hat{\mathcal{F}} (x_t), \hat{\mathcal{K}}_x (x_t), \hat{\mathcal{K}_y} (y_t)) \equiv (\mathcal{F} (x_t, \xi_{t}), \mathcal{K}_x (x_t, \xi_{t}), \mathcal{K}_y (y_t, \xi_{t}))$, where $\{\xi_t\}_{t \ge 1}$ is a sequence of i.i.d. random variables independent of $(x_t,y_t)$. Further assume that 
\begin{align}\label{eqn:expect}
\expect[\hat{\mathcal{F}}(x_i)] = \nabla f(x_i), \;\; \expect \left[\begin{pmatrix}- \hat{\mathcal{K}}_x (x_i) \\ \hat{\mathcal{K}}_y (y_i)\end{pmatrix} \right] = \begin{pmatrix}-Kx_i \\ K^T y_i \end{pmatrix}, \\
\expect[\hat{\mathcal{A}}(x_i)] = Ax_i,\;\; \text{and} \;\; \expect[\hat{\mathcal{B}}(y_i)] = B^T y_i
\end{align}
and 
\begin{align}\label{eqn:A1}
\expect[\|\hat{\mathcal{F}} - \nabla f(x_t) \|^2] \le \sigma_{x, f}^2, \;\; \expect[\|\hat{\mathcal{K}}_x(x_t)-K x_t\|^2] \le \sigma_y^2, \expect[\|\hat{\mathcal{K}}_y(y_t) - K^T y_t\|^2] \le \sigma_{x, K}^2, \\
\expect[\|\hat{\mathcal{A}}(x_t)-A x_t\|^2] \le \sigma_A^2 \text{ and } \expect[\|\hat{\mathcal{B}}(y_t)-B^T y_t\|^2] \le \sigma_y^2.
\end{align}
For notational convenience, we denote $\sigma_x := \sqrt{\sigma_{x, f}^2 + \sigma_{x, K}^2}$. a lower bound on the rate of convergence for this problem is given by 
\begin{align}
\Omega \left(\frac{L_f}{N^2}+\frac{L_K}{N}+\frac{\sigma_x + \sigma_y}{\sqrt{N}}\right). 
\end{align}

We consider the following iteration:

\begin{subequations}\label{eqn:stocgen}
\begin{align}
\overline{u}_t &= \hat{\mathcal{K}}_x (x_t) - \theta_t \hat{\mathcal{A}}(x_t - x_{t-1}) \\
\overline{v}_t &= \hat{\mathcal{K}}_y (y_t+\frac{\theta_t\eta_{t-1}}{\eta_t}) + \hat{\mathcal{B}}\left(\left(\frac{\eta_{t-1}}{\eta_t}-1 \right) (y_t - y_{t-1})\right)\\
x_t^{md} &= (1-\beta_t^{-1})x_t^{ag} +\beta_t^{-1}x_t \label{eqn:stocgen:xtilde} \\
\tilde{u}_{t+1} &= \overline{u}_t - \eta_t(\hat{\mathcal{K}_x} + \hat{\mathcal{A}}) (\hat{\mathcal{F}}(x_t^{md}) + \overline{v}_{t}) \\
y_{t+1} &= \prox_{\tau_t h^*} (y_t + \tau_t \tilde{u}_{t+1}) \\
\tilde{v}_{t+1} &= \hat{\mathcal{K}}_y (y_{t+1}) +\hat{\mathcal{B}}(y_{t+1}-y_t - \theta_t (y_t - y_{t-1})) \\
x_{t+1} &= x_t - \eta_t (\hat{\mathcal{F}}(x_t^{md}) +  \tilde{v}_{t+1}) \\
x_{t+1}^{ag} &= (1 - \beta_t^{-1}) x_t^{ag} + \beta_t^{-1}x_{t+1} \\
y_{t+1}^{ag} &= (1 - \beta_t^{-1}) y_t^{ag} + \beta_t^{-1}y_{t+1}.
\end{align}
\end{subequations}

\subsection{Convergence Results}
We establish the expected rate of convergence for both bounded and unbounded cases, in terms of $g$ or $\tilde{g}$. Furthermore, in the bounded case with $A = -K$ and $B = bK$, in probability convergence is shown under the following ``light-tail'' assumption on $\mathcal{SO}$.
\begin{subequations}\label{eqn:A2}
\begin{align}
\expect \left[\exp(\|\nabla f(x)-\hat{\mathcal{F}}(x) \|^2/ \sigma_{x, f}^2) \right] &\le \exp(1) \\
\expect \left[\exp (\|Kx - \hat{\mathcal{K}}_x (x)\|^2/\sigma_y^2) \right] &\le \exp(1) \\
\expect \left[\exp (\|K^T y - \hat{\mathcal{K}}_y (y)\|^2/ \sigma_{x, K}^2 )\right] & \le \exp(1)
\end{align}
\end{subequations}
Note that \eqref{eqn:A2} implies \eqref{eqn:A1} by Jensen's inequality. 


\textbf{Bounded Case.}

The following summarizes the convergnece properties of \eqref{eqn:stocgen} when $Z$ is bounded. 

\begin{theorem}\label{thm:stocbdd}
Assume that \eqref{eqn:bdd} holds, for some $\Omega_X$, $\Omega_y$ $>0$. Also suppose that for all $t \ge 1$, the parameters $\beta_t$, $\theta_t$, $\eta_t$, and $\tau_t$ satisfy \eqref{eqn:betacondgen}, \eqref{eqn:thetacondbddgen}, 
\begin{subequations}\label{eqn:stocparam}
\begin{align}
\frac{r-p}{\eta_t} - \frac{L_f}{\beta_t} - \frac{L_A^2 \tau_t}{q} & \ge 0, \text{ and}\label{eqn:stoccond1}\\ 
\frac{s - q}{ \tau_t}- \eta_t\left(2 L_{K+A}L_{K+B} + \frac{L_B^2}{p}\right) & \ge 0 \label{eqn:stoccond2}
\end{align}
\end{subequations}
for some $p$, $q$, $r$, $s \in (0,1)$. Then, 

\begin{enumerate}[label=(\roman*)]
\item Under \eqref{eqn:A1}, for all $t \ge 1$, 
\begin{align}
\expect [g(z_{t+1}^{ag})] \le \mathcal{Q}_0(t),
\end{align}
where 
\begin{align}
\mathcal{Q}_0 (t) & := \frac{1}{\beta_t \gamma_t} (\frac{2\gamma_t}{\eta_t} \Omega_X^2 + \frac{2 \gamma_t}{\tau_t} \Omega_Y^2 ) + \frac{1}{2\beta_t \gamma_t} \sum_{i=1}^t (\frac{(2-r) \eta_i \gamma_i}{1-r} (\sigma_x^2 + \sigma_B^2) \\ \nonumber
&+\frac{(2-s) \tau_i \gamma_i}{1-s}(\sigma_y^2 + \sigma_A^2 + \eta_t^2 L_{K+A}^2 (\sigma_x^2 + \sigma_B^2)) )
\end{align}
\item Let $A=-K$ and $B=bK$. Then under \eqref{eqn:A2}, for all $\lambda>0$ and $t \ge 1$, 
\begin{align}
\prob (g(z_{t+1}^{ag})>\mathcal{Q}'_0(t) + \lambda \mathcal{Q}_1(t)) \le 3 \exp(-\lambda^2/3)+ 3 \exp(-\lambda), 
\end{align}
where
\begin{align}
\mathcal{Q}'_0 (t) & := \frac{1}{\beta_t \gamma_t} (\frac{2\gamma_t}{\eta_t} \Omega_X^2 + \frac{2 \gamma_t}{\tau_t} \Omega_Y^2 ) + \frac{1}{2\beta_t \gamma_t} \sum_{i=1}^t (\frac{(2-r) \eta_i \gamma_i}{1-r} \sigma_x^2 \\ \nonumber
&+\frac{(2-s) \tau_i \gamma_i}{1-s}\sigma_y^2  )
\end{align}
\begin{align}
\mathcal{Q}_1 (t) &:= \frac{1}{\beta_t \gamma_t} (\sqrt{2}\sigma_x \Omega_X+ \sigma_y \Omega_Y ) \sqrt{2 \sum_{i=1}^t \gamma_i^2 } + \frac{1}{2 \beta_t \gamma_t}\sum_{i=1}^t (\frac{(2-r) \eta_i \gamma_i}{1-r}\sigma_x^2  \\ \nonumber
&+ \frac{(2-s) \tau_i \gamma_i}{1-s} \sigma_y^2).
\end{align}
\end{enumerate}
\end{theorem}

\begin{corollary}\label{cor:stocbdd}
Assume the condition \eqref{eqn:bdd} holds. In Algorithm \eqref{eqn:stocgen}, if $N \ge 1$ is given, $A=-K$, $B=bK$,   and the parameters are set to 
\begin{align}
\beta_t & = \frac{t+1}{2},\;\;\theta_t = \frac{t-1}{t}, \eta_t = \frac{\Omega_X t}{2P L_f \Omega_X + Q L_K \Omega_Y (N-1) + S\sigma_x N \sqrt{N-1}}, \\
\tau_t &= \frac{\Omega_Y t }{R L_K \Omega_X (N-1) + T \sigma_y N \sqrt{N-1}}
\end{align}
where $P$, $Q$, $R$, $S$, and $T>0$ satisfies 
\begin{align}\label{eqn:stocbddparamcond}
P = \frac{1}{r-p}, QR \ge \max\left\{\frac{1}{r-p}, \frac{|b|^2/p}{s-q}\right\}, 
\end{align}
the following holds.

\begin{enumerate}[label=(\roman*)]
\item Under assumption \eqref{eqn:A1}, $\expect[g(z_N^{ag}] \le \mathcal{C}_0(N)$ where $\mathcal{C}_0(N)$ is  $\mathcal{O}\left( \frac{L_f}{N^2} + \frac{L_K}{N} + \frac{\sigma_x + \sigma_y}{\sqrt{N}}\right)$.
\item Under assumption \eqref{eqn:A2}, then for all $\lambda>0$, we have 
\begin{align}
P(g(z_N^{ag} > \mathcal{C}_0(N) + \lambda \mathcal{C}_1(N)) \le 3 \exp(-\lambda^2/3) + 3 \exp(- \lambda),
\end{align}
where $\mathcal{C}_1(N) = \mathcal{O}\left(\frac{\sigma_x + \sigma_y}{\sqrt{N}} \right)$.
\end{enumerate}
\end{corollary}

\textbf{Unbounded Case.}

For unbounded feasible set $Z$, we have the following theorem. 

\begin{theorem}\label{thm:stocunbdd}
Assume that $\{z_t^{ag}\} = \{(x_t^{ag}, y_t^{ag})\}$ is the iterates generated by \eqref{eqn:stocgen}. Furthere assume that the parameters $\beta_t$, $\theta_t$, $\eta_t$, and $\tau_t$ in \eqref{eqn:stocgen} satisfy \eqref{eqn:betacondgen}, \eqref{eqn:thetacondgen}, and \eqref{eqn:stocparam} for all $t \ge 1$ and some $p$, $q$, $r$, $s \in (0,1)$. Then there is a perterbation vector $v_{t+1}$ satisfying 
\begin{align}
\expect [\tilde{g}(z_{t+1}^{ag}, v_{t+1})] \le \frac{1}{\beta_t \eta_t} \left[ \left( 6 +\frac{4p}{1-p} +\frac{4(q+1/2)}{1/2-q}\right) D^2 + \left( \frac{5}{2} + \frac{2p}{1-p} + \frac{2(q+1/2)}{1/2-q} \right) C^2\right]
\end{align}
for all $t \ge 1$. Furthermore, 
\begin{align}
\expect[\|v_{t+1}\|] & \le \frac{2 \|\hat{x} - x_1\|}{\beta_t \eta_t}+ \frac{2 \|\hat{y}-y_1\|}{\beta_t \tau_t} + \sqrt{2D^2+C^2} [\frac{1+\mu}{\beta_t \eta_t} +(\nu + \sqrt{\frac{\tau_1}{\eta_1}}) \frac{1}{\beta_t \tau_t} \\
&+ \frac{2}{\beta_t} (L_A\mu + L_B\nu ) + \frac{2 \eta_t}{\beta_t}L_{K+A}L_{K+B} \nu ] =: \epsilon_{t+1}
\end{align}
where $(\hat{x}, \hat{y})$ is a pair of solutions for \eqref{eqn:saddle}, $D$, $\mu$, and $\nu$ are defined in \eqref{eqn:Ddefgen}, and 
\begin{align}\label{eqn:Cdef}
C &:= \sqrt{\sum_{i=1}^t \frac{(2-r)\eta_i^2 (\sigma_x^2+\sigma_B^2)}{1-r} + \sum_{i=1}^t \frac{(2-s)\eta_i \tau_i (\sigma_y^2 + \sigma_A^2 + \eta_t^2 L_{K+A}^2 (\sigma_x^2 + \sigma_B^2))}{1-s}}.
\end{align}
\end{theorem}


\begin{corollary}\label{cor:stocunbdd}
In Algorithm \eqref{eqn:stocgen}, if $N$ is given, $A=-K$, $B=bK$, and the paramters are set to 
\begin{align}
\beta_t = \frac{t+1}{2}, \;\; \theta_t = \frac{t-1}{t}, \;\; \eta_t = \frac{t}{\eta}, \;\; \tau_t = \frac{R t}{\eta},
\end{align}
where 
\begin{align}
\eta = 2 P L_f + 2 Q L_K (N-1) + S N \sqrt{N-1} \sigma/\tilde{D}
\end{align}
for some $\tilde{D}>0$, where $\sigma$ is defined by $\sigma = \sqrt{\frac{2-r}{1-r} 2\sigma_x^2 + w \frac{2-s}{1-s} 2\sigma_y^2}$. 
Then for $P$, $Q$, $R$, and $S$ satisfying 
\begin{align}\label{eqn:stocunbddparamcond}
P = \frac{1}{r-p},\;\; Q^2 \ge \max \left\{ \frac{|a|^2 R}{4q(r - p)}, \frac{(|b|^2/p)R}{4(s - q)}\right\},
\end{align}
then both $\epsilon_N$ and $\expect[\|v_N\|]$ are $\mathcal{O}\left(\frac{L_f}{N^2}+\frac{L_K}{N}+ \frac{\sigma}{\sqrt{N}}\right)$. 
\end{corollary}

\begin{remark}
Corollaries \ref{cor:stocbdd} and \ref{cor:stocunbdd} only admits the cases with $A=-K$. i.e., The variants of Algorithm CV are guaranteed the optimal rate, but the variants of Algorithm LV are not. However, Algorithm LV shows similar behavior to Algorithm CV in our numerical experiments.
\end{remark}








